Lepton-flavour-violating gluonic operators: constraints from the LHC and low energy experiments

Effective operators provide a model-independent description of physics beyond the stan- dard model that is particularly useful given the absence of any signs of new physics at the Large Hadron Collider (LHC). We recast previous LHC analyses to set limits on lepton-flavour-violating gluonic effective operators of dimension 8 and compare our results to existing limits from low-energy precision experiments. Current LHC data constrains the scale $\Lambda$ of the effective operators to be larger than $\Lambda\gtrsim 0.5 - 1.6$ TeV depending on the flavour and thus provides the most stringent limit for all operators apart from parity-conserving operators of the form $GG\bar\mu P_{L,R} e$, where $\mu - e$ conversion in nuclei poses the most stringent constraint.

==> tikzfeynman.keys.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TikZ-Feynman
% Feynman Diagrams with TikZ
% Copyright (C) 2015  Joshua Ellis
%
%
% This work may be distributed and/or modified under the conditions of the LaTeX
% Project Public License, either version 1.3 of this license or (at your option)
% any later version.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Joshua Ellis.
%
% This program is distributed in the hope that it will be useful, but WITHOUT
% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE.  See the LaTeX Project Public License for more
% details.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Shapes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Crossed Circle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{crossed circle}
{
  \inheritsavedanchors[from=circle]
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}

  \inheritbackgroundpath[from=circle]

  \foregroundpath{
    % Compute south west
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by-0.707107\pgf@xc
    \advance\pgf@y by-0.707107\pgf@xc
    \pgf@xa=\pgf@x \pgf@ya=\pgf@y  % Store coordinates
    % Compute north east point
    \centerpoint
    \pgf@xc=\radius
    \advance\pgf@x by0.707107\pgf@xc
    \advance\pgf@y by0.707107\pgf@xc
    \pgf@xb=\pgf@x \pgf@yb=\pgf@y  % Store coordinates
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfsetarrowsstart{}
    \pgfsetarrowsend{}
 }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Decorations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete Sines
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Complete sines replaces the path with a whole number of sine waves.
%% Thanks to http://tex.stackexchange.com/a/134516/26980
\pgfdeclaredecoration{complete sines}{initial}
{
  %% Begin by computing the overall path length and find how many sine waves we
  %% can fit in.  Nothing happens beyond the computation.
  \state{initial}[
    width=+0pt,
    next state=move,
    persistent precomputation={
      \def\tikzfeynman@cs@angle@step{30}
      \def\tikzfeynman@cs@current@angle{0}
      \pgfmathsetlengthmacro{\tikzfeynman@cs@points@per@step}{
        \pgfdecoratedinputsegmentlength
        / int(\pgfdecoratedinputsegmentlength
        / \pgfdecorationsegmentlength)
        / 360
        * \tikzfeynman@cs@angle@step}
    },
  ]{}
  %% Move to the origin to the path
  \state{move}[
    width=+\tikzfeynman@cs@points@per@step,
    next state=draw
  ]{
    \pgfpathmoveto{\pgfpointorigin}
  }
  %% Draw the sine wave itself.  This computes the value every 20 degrees and draws straight edges.
  \state{draw}[
    width=+\tikzfeynman@cs@points@per@step,
    switch if less than=1.25*\tikzfeynman@cs@points@per@step to final, % <- bit of a hack
    persistent postcomputation={
      \pgfmathparse{mod(\tikzfeynman@cs@current@angle+\tikzfeynman@cs@angle@step, 360)}
      \let\tikzfeynman@cs@current@angle=\pgfmathresult%
    },
  ]{
    \pgfmathparse{sin(\tikzfeynman@cs@current@angle) * \pgfmetadecorationsegmentamplitude / 2}
    \tikz@decoratepathfalse
    \pgfpathlineto{\pgfqpoint{0pt}{\pgfmathresult pt}}%
  }

  \state{final}{
    \ifdim\pgfdecoratedremainingdistance>0pt\relax
      \pgfpathlineto{\pgfpointdecoratedpathlast}
    \fi
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Keys
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzfeynmanset{
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Hooks
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  execute at begin feynman/.code={},
  execute at end feynman/.code={},
  every feynman/.style={/tikzfeynman/every feynman@@/.append style={#1}},
  every feynman@@/.style={
    /tikzfeynman/.cd,
    /tikzfeynman/medium,
  },
  execute at begin feynman@@/.code={}                     %% Internal version
  execute at end feynman@@/.code={},                      %% Internal version
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Diagrams
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every diagram/.style={/tikzfeynman/every diagram@@/.append style={#1}},
  every diagram@@/.style={
    /tikzfeynman/.cd,
    .search also={/tikz/graphs, /tikz},
    nodes={
      /tikzfeynman/.cd,
      /tikzfeynman/.search also={/tikz/graphs, /tikz},
      /tikzfeynman/every vertex@@,
      /tikzfeynman/every vertex},
    edges={
      /tikzfeynman/.cd,
      /tikzfeynman/.search also={/tikz/graphs, /tikz},
      /tikzfeynman/every edge@@,
      /tikzfeynman/every edge},
    /tikzfeynman/medium,
  },
  every inline/.style={/tikzfeynman/inline@@/.append style={#1}},
  every inline@@/.style={
    /tikzfeynman/small,
  },
  inline/.style={
    /tikz/baseline={#1},
    /tikzfeynman/every inline@@,
  },
  every small/.style={/tikzfeynman/small@@/.append style={#1}},
  every small@@/.style={
    /tikz/node distance=1cm,
    /graph drawing/node distance=1.25cm,
    /graph drawing/level distance=1cm,
    /graph drawing/sibling distance=1.5cm,
    /tikzfeynman/every dot@@/.append style={/tikz/minimum size=1mm},
    /tikzfeynman/every crossed dot@@/.append style={/tikz/minimum size=2mm},
    /tikzfeynman/every blob@@/.append style={/tikz/minimum size=0.5cm},
    /tikzfeynman/arrow size=1.2pt,
    /tikzfeynman/insertion/size=2.5pt,
  },
  small/.style={/tikzfeynman/every small@@},
  every medium/.style={/tikzfeynman/medium@@/.append style={#1}},
  every medium@@/.style={
    /tikz/node distance=1.5cm,
    /graph drawing/node distance=1.9cm,
    /graph drawing/level distance=1.5cm,
    /graph drawing/sibling distance=2.25cm,
  },
  medium/.style={/tikzfeynman/every medium@@},
  every large/.style={/tikzfeynman/large@@/.append style={#1}},
  every large@@/.style={
    /tikz/node distance=2cm,
    /graph drawing/node distance=2.5cm,
    /graph drawing/level distance=2cm,
    /graph drawing/sibling distance=3cm,
    /tikz/graphs/edges={thick},
    /tikzfeynman/every dot@@/.append style={/tikz/minimum size=2mm},
    /tikzfeynman/every crossed dot@@/.append style={/tikz/minimum size=4mm},
    /tikzfeynman/every blob@@/.append style={/tikz/minimum size=1cm},
    /tikzfeynman/arrow size=1.6pt,
    /tikzfeynman/insertion/size=4pt,
  },
  large/.style={/tikzfeynman/every large@@},
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Vertices
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every vertex@@/.style={
    /tikz/shape=coordinate,
  },
  every vertex/.style={/tikzfeynman/every vertex@@/.append style={#1}},
  vertex/.style={
    /tikzfeynman/every vertex@@,
  },
  every dot@@/.style={
    /tikz/shape=circle,
    /tikz/graphs/as={},
    /tikz/draw,
    /tikz/fill,
    /tikz/inner sep=0pt,
    /tikz/outer sep=0pt,
    /tikz/minimum size=1.5mm,
  },
  every dot/.style={/tikzfeynman/every dot@@/.append style={#1}},
  dot/.style={
    /tikzfeynman/every dot@@,
  },
  every square dot@@/.style={
    /tikz/shape=rectangle,
  },
  every square dot/.style={/tikzfeynman/every square dot@@/.append style={#1}},
  square dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every square dot@@,
  },
  every empty dot@@/.style={
    /tikz/fill=none,
  },
  every empty dot/.style={/tikzfeynman/every empty dot@@/.append style={#1}},
  empty dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every empty dot@@,
  },
  every crossed dot@@/.style={
    /tikz/fill=none,
    /tikz/shape=crossed circle,
    /tikz/minimum size=3mm,
  },
  every crossed dot/.style={/tikzfeynman/every crossed dot@@/.append style={#1}},
  crossed dot/.style={
    /tikzfeynman/every dot@@,
    /tikzfeynman/every crossed dot@@,
  },
  every blob@@/.style={
    /tikz/shape=circle,
    /tikz/graphs/as={},
    /tikz/draw,
    /tikz/fill=none,
    /tikz/outer sep=0.5\pgflinewidth,
    /tikz/inner sep=0pt,
    /tikz/minimum size=0.75cm,
    /tikz/pattern=north west lines,
  },
  every blob/.style={/tikzfeynman/every blob@@/.append style={#1}},
  blob/.style={
    /tikzfeynman/every blob@@,
  },
  every particle@@/.style={
    /tikz/shape=rectangle,
    /tikz/draw=none,
    /tikz/fill=none,
    /tikz/inner sep=0.3333em,
    /tikz/outer sep=0.5\pgflinewidth,
  },
  every particle/.style={/tikzfeynman/every particle@@/.append style={#1}},
  particle/.style args={#1}{
    /tikzfeynman/every particle@@,
    /tikz/graphs/as={#1},
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Edge styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Arrow Style
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  arrow size/.store in=\tikzfeynman@arrow@size,
  arrow size=1.5pt,
  with arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          xshift=-0.5mm,
          fill,
          inner sep=\tikzfeynman@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  with reversed arrow/.style={
    /tikz/decoration={
      markings,
      mark=at position #1 with {
        \node[
          transform shape,
          xshift=-0.5mm,
          rotate=180,
          fill,
          inner sep=\tikzfeynman@arrow@size,
          draw=none,
          isosceles triangle
        ] { };
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  %% Base Edge Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every edge@@/.style={},
  every edge/.style={/tikzfeynman/every edge@@/.append style={#1}},
  %% Specific Styles
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  every plain@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw
    },
  },
  every plain/.style={/tikzfeynman/every plain@@/.append style={#1}},
  plain/.style={
    /tikzfeynman/every plain@@,
  },
  every boson@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        complete sines,
        amplitude=1mm,
        segment length=2mm,
      },
      /tikz/decorate=true,
    },
  },
  every boson/.style={/tikzfeynman/every boson@@/.append style={#1}},
  boson/.style={
    /tikzfeynman/every boson@@,
  },
  every charged boson@@/.style={
    /tikzfeynman/with arrow=0.5,
  },
  every charged boson/.style={/tikzfeynman/every charged boson@@/.append style={#1}},
  charged boson/.style={
    /tikzfeynman/boson,
    /tikzfeynman/every charged boson@@,
  },
  every anti charged boson@@/.style={
    /tikzfeynman/with reversed arrow=0.5,
  },
  every anti charged boson/.style={/tikzfeynman/every anti charged boson@@/.append style={#1}},
  anti charged boson/.style={
    /tikzfeynman/boson,
    /tikzfeynman/every anti charged boson@@,
  },
  every photon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        complete sines,
        amplitude=1mm,
        segment length=2mm,
      },
      /tikz/decorate=true,
    },
  },
  every photon/.style={/tikzfeynman/every photon@@/.append style={#1}},
  photon/.style={
    /tikzfeynman/every photon@@,
  },
  every scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dashed,
    },
  },
  every scalar/.style={/tikzfeynman/every scalar@@/.append style={#1}},
  scalar/.style={
    /tikzfeynman/every scalar@@,
  },
  every charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynman/with arrow=0.5,
    },
  },
  every charged scalar/.style={/tikzfeynman/every charged scalar@@/.append style={#1}},
  charged scalar/.style={
    /tikzfeynman/scalar,
    /tikzfeynman/every charged scalar@@,
  },
  every anti charged scalar@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikzfeynman/with reversed arrow=0.5,
    },
  },
  every anti charged scalar/.style={/tikzfeynman/every anti charged scalar@@/.append style={#1}},
  anti charged scalar/.style={
    /tikzfeynman/scalar,
    /tikzfeynman/every anti charged scalar@@,
  },
  every ghost@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/dotted,
      /tikz/thick,
    },
  },
  every ghost/.style={/tikzfeynman/every ghost@@/.append style={#1}},
  ghost/.style={
    /tikzfeynman/every ghost@@,
  },
  every fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with arrow=0.5,
    },
  },
  every fermion/.style={/tikzfeynman/every fermion@@/.append style={#1}},
  fermion/.style={
    /tikzfeynman/every fermion@@,
  },
  every anti fermion@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with reversed arrow=0.5,
    },
  },
  every anti fermion/.style={/tikzfeynman/every anti fermion@@/.append style={#1}},
  anti fermion/.style={
    /tikzfeynman/every anti fermion@@,
  },
  every majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with arrow=0.33,
      /tikzfeynman/with reversed arrow=0.73,
    },
  },
  every majorana/.style={/tikzfeynman/every majorana@@/.append style={#1}},
  majorana/.style={
    /tikzfeynman/every majorana@@,
  },
  every anti majorana@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikzfeynman/with reversed arrow=0.33,
      /tikzfeynman/with arrow=0.73,
    },
  },
  every anti majorana/.style={/tikzfeynman/every anti majorana@@/.append style={#1}},
  anti majorana/.style={
    /tikzfeynman/every anti majorana@@,
  },
  every gluon@@/.style={
    /tikz/draw=none,
    /tikz/decoration={name=none},
    /tikz/postaction={
      /tikz/draw,
      /tikz/decoration={
        coil,
        aspect=0.75,
        mirror,
        segment length=1.5mm
      },
      /tikz/decorate=true,
    },
  },
  every gluon/.style={/tikzfeynman/every gluon@@/.append style={#1}},
  gluon/.style={
    /tikzfeynman/every gluon@@,
  },
  %% Insertions
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  insertion/.search also={/tikzfeynman,/tikz},
  %% Parameters
  insertion/size/.store in=\tikzfeynman@insertion@size,
  insertion/size=3pt,
  insertion/style/.store in=\tikzfeynman@insertion@style,
  insertion/style={},
  %% Styles
  insertion@@/.style args={[#1]#2}{
    /tikz/decoration={
      markings,
      mark=at position #2 with {
        \tikzfeynmanset{insertion/.cd,#1}
        \draw [\tikzfeynman@insertion@style] (-\tikzfeynman@insertion@size, -\tikzfeynman@insertion@size) -- (\tikzfeynman@insertion@size, \tikzfeynman@insertion@size);
        \draw [\tikzfeynman@insertion@style] (-\tikzfeynman@insertion@size, \tikzfeynman@insertion@size) -- (\tikzfeynman@insertion@size, -\tikzfeynman@insertion@size);
      },
    },
    /tikz/postaction={
      /tikz/decorate=true,
    },
  },
  insertion@@/.default={[]0.5},
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Momentum arrows
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  momentum/.search also={/tikzfeynman,/tikz},
  %% Parameters
  momentum/label distance/.store in=\tikzfeynman@momentum@label@distance,
  momentum/label distance=0pt,
  momentum/arrow distance/.store in=\tikzfeynman@momentum@arrow@distance,
  momentum/arrow distance=3mm,
  momentum/arrow shorten/.store in=\tikzfeynman@momentum@arrow@shorten,
  momentum/arrow shorten=0.15,
  momentum/label style/.store in=\tikzfeynman@momentum@label@style,
  momentum/label style={},
  momentum/arrow style/.store in=\tikzfeynman@momentum@arrow@style,
  momentum/arrow style={},
  %% Styles
  momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst)
                .. controls (\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
                .. (\tikzinputsegmentlast)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentfirst) -- (\tikzinputsegmentlast)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@26)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@1)$)
                node [pos=0.5, auto, swap,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  reversed momentum'@@/.style args={[#1]#2}{
    /tikz/preaction={
      /tikz/decoration={
        show path construction,
        moveto code={},
        lineto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
        curveto code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast)
                .. controls (\tikzinputsegmentsupportb) and (\tikzinputsegmentsupporta)
                .. (\tikzinputsegmentfirst)
                { \foreach \i in {1, ..., 50} {
                  coordinate [pos=\tikzfeynman@momentum@arrow@shorten + (1-2 * \tikzfeynman@momentum@arrow@shorten)*\i/50] (tf@m@\i) } };
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                foreach \i [count=\j from 3] in {2, ..., 24} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@25)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@26)$)
                node [pos=0.5,
                      auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@arrow@style] {#2}
                foreach \i [count=\j from 27] in {26, ..., 49} {
                  -- ($(tf@m@\i)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@\j)$)
                }
                -- ($(tf@m@50)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@49)$);
        },
        closepath code={
          \tikzfeynmanset{momentum/.cd,#1}
          \path (\tikzinputsegmentlast) -- (\tikzinputsegmentfirst)
                coordinate [pos=\tikzfeynman@momentum@arrow@shorten] (tf@m@1)
                coordinate [pos=1 - \tikzfeynman@momentum@arrow@shorten] (tf@m@2);
          \draw [-Stealth, \tikzfeynman@momentum@arrow@style]
                ($(tf@m@1)!\tikzfeynman@momentum@arrow@distance!90:(tf@m@2)$)
                -- ($(tf@m@2)!\tikzfeynman@momentum@arrow@distance!-90:(tf@m@1)$)
                node [pos=0.5, auto,
                      outer sep=\tikzfeynman@momentum@label@distance,
                      \tikzfeynman@momentum@label@style] {#2};
        },
      },
      /tikz/decorate=true,
    },
  },
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %% Modifiers
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  half left/.style={
    /tikz/bend left=90,
    /tikz/looseness=1.5,
  },
  half right/.style={
    /tikz/bend right=90,
    /tikz/looseness=1.5,
  },
  quarter left/.style={
    /tikz/bend left=45,
  },
  quarter right/.style={
    /tikz/bend right=45,
  },
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Graceful Failure of LuaTeX keys
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@luatex@required@path{
  \PackageWarning{tikz-feynman}{The key you tried to use '\pgfkeyscurrentpath/\pgfkeyscurrentname' requires LuaTeX.  It will be ignored.}
}
\def\tikzfeynman@luatex@required@key{
  \PackageWarning{tikz-feynman}{The key you tried to use '\pgfkeyscurrentpath' requires LuaTeX.  It will be ignored.}
}

\ifluatex\else
  \pgfkeys{
    /graph drawing/.unknown/.code=\tikzfeynman@luatex@required@path,
    /tikz/graphs/.unknown/.code=\tikzfeynman@luatex@required@path,
    /tikz/horizontal/.code=\tikzfeynman@luatex@required@key,
    /tikz/horizontal'/.code=\tikzfeynman@luatex@required@key,
    /tikz/vertical/.code=\tikzfeynman@luatex@required@key,
    /tikz/vertical'/.code=\tikzfeynman@luatex@required@key,
    /tikz/tree layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/spring layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/layered layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/spring electrical layout/.code=\tikzfeynman@luatex@required@key,
    /tikz/electric charge/.code=\tikzfeynman@luatex@required@key,
  }
  % \tikzfeynmanset{
  %   horizontal/.code={The key 'horizontal' requires LuaTeX.  It will be ignored.},
  % }
\fi

\endinput

==> tikzlibraryfeynman.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% TikZ-Feynman
% Feynman Diagrams with TikZ
% Copyright (C) 2015  Joshua Ellis
%
%
% This work may be distributed and/or modified under the conditions of the LaTeX
% Project Public License, either version 1.3 of this license or (at your option)
% any later version.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Joshua Ellis.
%
% This program is distributed in the hope that it will be useful, but WITHOUT
% ANY WARRANTY; without even the implied warranty of MERCHANTABILITY or FITNESS
% FOR A PARTICULAR PURPOSE.  See the LaTeX Project Public License for more
% details.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Pre-requisites
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usetikzlibrary{
  arrows.meta,
  calc,
  decorations,
  decorations.markings,
  decorations.pathmorphing,
  decorations.pathreplacing,
  graphs,
  patterns,
  positioning,
  shapes.geometric,
}
\ifluatex
  \usetikzlibrary{
    graphdrawing
  }
  \usegdlibrary{
    circular,
    force,
    layered,
    trees
  }
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Function definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Miscellaneous functions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@empty{}

%% Key Manager
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Setup the tikz-feynman key family
\pgfkeys{
  /tikzfeynman/.is family,
  /tikzfeynman/.search also={/tikz},
}

%% |\tikzfeynmanset| allows keys that belong with tikz-feynman to be easily set.
\def\tikzfeynmanset{\pgfqkeys{/tikzfeynman}}

%% Luatex Waring
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Check if we are using luatex
\newif\iftikzfeynman@warn@luatex%
\tikzfeynmanset{
  warn luatex/.is if=tikzfeynman@warn@luatex,
  warn luatex=true,
}

\AtBeginDocument{
  \ifluatex\else
    \iftikzfeynman@warn@luatex
      \PackageWarning{tikz-feynman}{LuaTeX is required if you wish to have vertices automatically placed.  You can disable this warning by setting /tikzfeynman/warn luatex=false}
    \fi
  \fi
}

%% Version check
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Check which version is expected and which is installed
\def\tikzfeynman@compat@parse#1.#2.#3\pgfeov{
  \edef\tikzfeynman@compat@major{#1}
  \edef\tikzfeynman@compat@minor{#2}
  \edef\tikzfeynman@compat@patch{#3}
  \edef\tikzfeynman@compat{#1.#2.#3}
}
\let\tikzfeynman@compat=\tikzfeynman@empty
\pgfkeyslet{/tikzfeynman/compat/.@cmd}{\tikzfeynman@compat@parse}
\ProcessPgfPackageOptions{/tikzfeynman}

\AtBeginDocument{
  \ifx\tikzfeynman@version\tikzfeynman@compat\else
    \ifx\tikzfeynman@compat\tikzfeynman@empty
      \PackageWarning{tikz-feynman}{Consider loading TikZ-Feynman with \string\usepackage[compat=\tikzfeynman@version]{tikz-feynman} so that you can be warned if TikZ-Feynman changes.}
    \else
      \ifx\tikzfeynman@compat@major\tikzfeynman@version@major
        \ifx\tikzfeynman@compat@minor\tikzfeynman@version@minor
          \ifx\tikzfeynman@compat@patch\tikzfeynman@version@patch\else
            \PackageInfo{tikz-feynman}{The preamble requested version \tikzfeynman@compat, but the system version is \tikzfeynman@version.  This should cause no issue.}
          \fi
        \else
          \PackageWarning{tikz-feynman}{The preamble requested version \tikzfeynman@compat, but the system version is \tikzfeynman@version.  This may change some diagrams.}
        \fi
      \else
        \PackageError{tikz-feynman}{The preamble requested version \tikzfeynman@compat, but the system version is \tikzfeynman@version.  They are most likely incompatible.  Please download the appropriate version from jpellis.me/projects/tikz-feynman.}
      \fi
    \fi
  \fi
}

%% Override Lua code if necessary
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@apply@patch#1{
  \directlua{require("tikzfeynman.patch.#1.lua")}
}

%% Version 3.0.0, 3.0.1 and 3.0.1a need to be patched.
\ifluatex
  \def\tikzfeynman@temp{3.0.0}
  \ifx\pgfversion\tikzfeynman@temp
    \tikzfeynman@apply@patch{3.0.0}
  \else
    \def\tikzfeynman@temp{3.0.1}
    \ifx\pgfversion\tikzfeynman@temp
      \tikzfeynman@apply@patch{3.0.1}
    \else
      \def\tikzfeynman@temp{3.0.1a}
      \ifx\pgfversion\tikzfeynman@temp
        \tikzfeynman@apply@patch{3.0.1}
      \fi
    \fi
  \fi
\fi

%% Feynman Environment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Provide `\begin{feynman} ... \end{feynman}` within TikZ pictures.
\tikzaddtikzonlycommandshortcutlet\feynman\tikzfeynman@environment@feynman
\tikzaddtikzonlycommandshortcutlet\endfeynman\endtikzfeynman@environment@feynman

%% \begin{feynman}...\end{feynman}
\def\tikzfeynman@environment@feynman{%
  \pgfutil@ifnextchar[{\tikzfeynman@environment@feynman@opt}
  {\tikzfeynman@environment@feynman@opt[]}}

\def\tikzfeynman@environment@feynman@opt[#1]{%
  \begingroup
  %% Local overrides
  \let\tikz@@scan@fig=\tikzfeynman@scan@fig
  \let\tikzfeynman@orig@graph=\graph
  %% Local commands
  \let\vertex=\tikzfeynman@commands@vertex
  \let\diagram=\tikzfeynman@commands@diagram
  \let\graph=\tikzfeynman@commands@graph
  %% Opening hooks
  \scope
  \tikz@lib@ignore@sizetrue
  \tikzfeynman@tikz@search@tikzfeynman
  \pgfkeys{/tikzfeynman/every feynman@@,#1}
  \pgfkeysvalueof{/tikzfeynman/execute at begin feynman@@}%
  \pgfkeysvalueof{/tikzfeynman/execute at begin feynman}%
}

\def\endtikzfeynman@environment@feynman{%
  %% Closing hooks
  \pgfkeysvalueof{/tikzfeynman/execute at end feynman}%
  \pgfkeysvalueof{/tikzfeynman/execute at end feynman@@}%
  \endscope
  \endgroup
}

%% \feynmandiagram
\def\feynmandiagram{%
  \pgfutil@ifnextchar[{\feynmandiagram@opt}
  {\feynmandiagram@opt[]}}
\def\feynmandiagram@opt[#1]{%
  \pgfutil@ifnextchar[{\feynmandiagram@opt@opt[#1]}
  {\feynmandiagram@opt@opt[#1][#1]}}
\def\feynmandiagram@opt@opt[#1][#2]{%
  \tikz [/tikzfeynman/.cd,#1]
  \graph [/tikzfeynman/.cd,/tikzfeynman/every diagram@@,/tikz/graphs/spring layout,#2]}

%% Allow empty nodes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\iftikzfeynmanallowemptynode
\newif\iftikzfeynmanvertex
\def\tikzfeynman@scan@fig{%
  \pgfutil@ifnextchar a{\tikz@fig@scan@at}
  {\pgfutil@ifnextchar({\tikz@fig@scan@name}
    {\pgfutil@ifnextchar[{\tikz@fig@scan@options}%
      {\pgfutil@ifnextchar\bgroup{\tikz@fig@main}%
      {\iftikzfeynmanvertex%
         \tikzset{/tikzfeynman/every vertex@@}%
         \iftikzfeynmanallowemptynode%
         \else%
           \tikzset{/tikzfeynman/particle}%
         \fi%
       \fi%
       \tikz@fig@main{}}}}}}%}}

%% Include /tikzfeynman in the search path
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@tikz@search@tikzfeynman{%
  \pgfkeys{/tikz/.unknown/.code=%
    \let\tikz@key\pgfkeyscurrentname%
    %% Is it a tikzfeynman key?
    \pgfkeys{/tikzfeynman/\tikz@key/.try={##1}}%
    \ifpgfkeyssuccess%
    \else%
      %% Is it a pgf key?
      \pgfkeys{/pgf/\tikz@key/.try={##1}}%
      \ifpgfkeyssuccess%
      \else%
        \expandafter\pgfutil@in@\expandafter!\expandafter{\tikz@key}%
        \ifpgfutil@in@%
          %% this is a color!
          \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
          \edef\tikz@textcolor{\tikz@key}%
        \else%
          \pgfutil@doifcolorelse{\tikz@key}
          {%
            \expandafter\tikz@addoption\expandafter{\expandafter\tikz@compat@color@set\expandafter{\tikz@key}}%
            \edef\tikz@textcolor{\tikz@key}%
          }%
          {%
            %% Ok, second chance: This might be an arrow specification:
            \expandafter\pgfutil@in@\expandafter-\expandafter{\tikz@key}%
            \ifpgfutil@in@%
              %% Ah, an arrow spec!
              \expandafter\tikz@processarrows\expandafter{\tikz@key}%
            \else%
              %% Ok, third chance: A shape!
              \expandafter\ifx\csname pgf@sh@s@\tikz@key\endcsname\relax%
                \pgfkeys{/errors/unknown key/.expand
                once=\expandafter{\expandafter/\expandafter t\expandafter
                i\expandafter k\expandafter z\expandafter/\tikz@key}{##1}}%
              \else%
                \edef\tikz@shape{\tikz@key}%
              \fi%
            \fi%
          }%
        \fi%
      \fi%
    \fi%
  }
}


%% Vertex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Adapted from |\coordinate| code
\def\tikzfeynman@commands@vertex{
  \path \pgfextra{\tikzfeynmanallowemptynodetrue}
        \pgfextra{\tikzfeynmanvertextrue}
        node}

%% Diagram
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@commands@diagram{\@ifstar
  \tikzfeynman@commands@diagram@star%
  \tikzfeynman@commands@diagram@nostar}

\def\tikzfeynman@commands@diagram@nostar{%
  \pgfutil@ifnextchar[{\tikzfeynman@commands@diagram@nostar@opt}
  {\tikzfeynman@commands@diagram@nostar@opt[]}}
\def\tikzfeynman@commands@diagram@nostar@opt[#1]{%
  \tikzfeynman@orig@graph [/tikzfeynman/every diagram@@,/tikz/graphs/spring layout,#1]}

\def\tikzfeynman@commands@diagram@star{%
  \pgfutil@ifnextchar[{\tikzfeynman@commands@diagram@star@opt}
  {\tikzfeynman@commands@diagram@star@opt[]}}
\def\tikzfeynman@commands@diagram@star@opt[#1]{%
  \tikzfeynman@orig@graph [/tikzfeynman/every diagram@@,#1]}

%% Graph
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@commands@graph{%
  \pgfutil@ifnextchar[{\tikzfeynman@commands@graph@opt}
  {\tikzfeynman@commands@graph@opt[]}}
\def\tikzfeynman@commands@graph@opt[#1]{%
  \PackageWarning{tikz-feynman}{It is not recommended to use \string\graph.  Use \string\diagram\space or \string\diagram* instead.}
  \tikzfeynman@orig@graph [/tikzfeynman/every diagram@@,#1]}

%% Optional argument in style key
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@key@opt#1[#2]#3\pgfeov{%
  \tikzfeynmanset{#1={[#2]#3}}}

%% Insertion
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@insertion{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{insertion@@}}
  {\tikzfeynman@key@opt{insertion@@}[]}}
\pgfkeyslet{/tikzfeynman/insertion/.@cmd}{\tikzfeynman@insertion}

%% Momentum
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tikzfeynman@momentum@std{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{momentum@@}}
  {\tikzfeynman@key@opt{momentum@@}[]}}
\pgfkeyslet{/tikzfeynman/momentum/.@cmd}{\tikzfeynman@momentum@std}

\def\tikzfeynman@momentum@stdp{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{momentum'@@}}
  {\tikzfeynman@key@opt{momentum'@@}[]}}
\pgfkeyslet{/tikzfeynman/momentum'/.@cmd}{\tikzfeynman@momentum@stdp}

\def\tikzfeynman@momentum@stdr{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{reversed momentum@@}}
  {\tikzfeynman@key@opt{reversed momentum@@}[]}}
\pgfkeyslet{/tikzfeynman/reversed momentum/.@cmd}{\tikzfeynman@momentum@stdr}
\pgfkeyslet{/tikzfeynman/rmomentum/.@cmd}{\tikzfeynman@momentum@stdr}

\def\tikzfeynman@momentum@stdrp{%
  \pgfutil@ifnextchar[{\tikzfeynman@key@opt{reversed momentum'@@}}
  {\tikzfeynman@key@opt{reversed momentum'@@}[]}}
\pgfkeyslet{/tikzfeynman/reversed momentum'/.@cmd}{\tikzfeynman@momentum@stdrp}
\pgfkeyslet{/tikzfeynman/rmomentum'/.@cmd}{\tikzfeynman@momentum@stdrp}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\input tikzfeynman.keys.code.tex

\endinput
